Base-pair mismatch can destabilize small DNA loops through cooperative kinking

Base pair mismatch can relieve mechanical stress in highly strained DNA molecules, but how it affects their kinetic stability is not known. Using single-molecule Fluorescence Resonance Energy Transfer (FRET), we measured the lifetimes of tightly bent DNA loops with and without base pair mismatch. Surprisingly, for loops captured by stackable sticky ends, the mismatch decreased the loop lifetime despite reducing the overall bending stress, and the decrease was largest when the mismatch was placed at the DNA midpoint. These findings show that base pair mismatch transfers bending stress to the opposite side of the loop through an allosteric mechanism known as cooperative kinking. Based on this mechanism, we present a three-state model that explains the apparent dichotomy between thermodynamic and kinetic stability of DNA loops.

==> sequences.tex <==
\begin{longtable}{|c|X|}
\hline

\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}l@{}}\textbf{DNA set 1 (5\textrm{$^\prime$} to 3\textrm{$^\prime$})}\end{tabular}}     \\ \hline
%\multicolumn{1}{|c|}{\textbf{First column}} & %\multicolumn{1}{c|}{\textbf{Third column}} \\ \hline 
\endfirsthead

%\multicolumn{2}{c}%
%{\tablename\ \thetable{} -- continued from previous page} \\
\hline 
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}l@{}}\textbf{DNA set 2 (5\textrm{$^\prime$} to 3\textrm{$^\prime$})} -- continued from previous page\end{tabular}}     \\ \hline
\endhead

\hline \multicolumn{2}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline
\caption{List of DNA sequences, PCR primers, and blocking oligonucleotides. All molecules in DNA sets 1 and 2 include the common adapter sequences (20 bp) at both ends, which are also present in the PCR primer pairs. PCR primers and blocking oligos are hybridized to each other to make the partial duplexes that are sticky on one end and blunt on the other: Blocking-Cy5full and Blocking-Cy5gap are hybridized with the forward primers of full and gapped sticky ends, and Blocking-Cy3 hybridizes with the backward primers of both full and gapped sticky ends, respectively. These partial duplexes are used to measure the association rate ($k_{\textrm{on}}$) between the sticky ends and the lifetime ($\tau_{\textrm{on}}$) of the linker duplex.
} \label{tab:sequences}
\endlastfoot

94 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCACCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTCCCATTCGAGCTCGTTGTAG}                       \\ \hline
96 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCATCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCCCATTCGAGCTCGTTGTAG}                     \\ \hline
98 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCATTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCCCCATTCGAGCTCGTTGTAG}                   \\ \hline
100 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCACCCATTCGAGCTCGTTGTAG}                 \\ \hline
102 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATCCCATTCGAGCTCGTTGTAG}               \\ \hline
104 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGCCCATTCGAGCTCGTTGTAG}             \\ \hline
106 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCATAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCCCATTCGAGCTCGTTGTAG}           \\ \hline
108 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCATTAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCCCCATTCGAGCTCGTTGTAG}         \\ \hline
110 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAGTTAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCACCCATTCGAGCTCGTTGTAG}       \\ \hline
112 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACGTTAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCAGCCCATTCGAGCTCGTTGTAG}     \\ \hline
114 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAGCGTTAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCAGGCCCATTCGAGCTCGTTGTAG}   \\ \hline
116 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAAGCGTTAACTTCCGGAGCCACACCGGTGCAAACCTCAGCAAGCAGGGTGTGGAAGTAGGACATTTTCATGTCAGGCCCCATTCGAGCTCGTTGTAG} \\ \hline

\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}l@{}}\textbf{DNA set 2 (5\textrm{$^\prime$} to 3\textrm{$^\prime$})}\end{tabular}}     \\ \hline

94 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCACATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATCCCATTCGAGCTCGTTGTTG}                       \\ \hline
108 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCACGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACACCCATTCGAGCTCGTTGTAG}                     \\ \hline
110 bp                  & \seqsplit{GTGCCAGCAACAGATAGCCAGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAACCCATTCGAGCTCGTTGTAG}                   \\ \hline
112 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATCCCATTCGAGCTCGTTGTAG}                 \\ \hline
114 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGCCCATTCGAGCTCGTTGTAG}               \\ \hline
116 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCATTCGAGCTCGTTGTAG}             \\ \hline
118 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCATTCGAGCTCGTTGTAG}           \\ \hline
120 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCCATTCGAGCTCGTTGTAG}         \\ \hline
122 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACCACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCCCATTCGAGCTCGTTGTAG}       \\ \hline
124 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACCCACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCCCCATTCGAGCTCGTTGTAG}     \\ \hline
153 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCAGGGGAAAGACCACACCCACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCGTTGCCACAGAGACCCCCATTCGAGCTCGTTGTAG}   \\ \hline
189 bp                 & \seqsplit{GTGCCAGCAACAGATAGCCACAGCAACGGGCAACCGTTTGGGGAAAGACCACACCCACGCGCGATCGCCATGGCAACGAGGTCGCACACGCCCCACACCCAGACCTCCCTGCGAGCGGGCATGGGTACAATGTCCCCGTTGCCACAGAGACCACTTCGTAGCACAGCGCCCCATTCGAGCTCGTTGTAG} \\ \hline

\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\bf Full sticky ends PCR primer pairs (5\textrm{$^\prime$} to 3\textrm{$^\prime$})\end{tabular}} \\ \hline
Forward                   & TGAATTTACG{[}Cy5dT{]}GCCAGCAACAGA{[}BiotindT{]}AGC
\\ \hline
Backward                  & GTAAATTCAC{[}Cy3dT{]}ACAACGAGCTCGAATGGG
\\ \hline
\multicolumn{2}{|c|}{\bf Gapped sticky ends PCR primer pairs (5\textrm{$^\prime$} to 3\textrm{$^\prime$})}                                           \\ \hline
Forward                   & TGAATTTACGCTG{[}Cy5dT{]}GCCAGCAACAGA{[}BiotindT{]}AGCCA                             \\ \hline
Backward                  & {[}Cy3{]}GTAAATTCACGACTACAACGAGCTCGAATGGG                 \\ \hline

\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}\bf Blocking oligos for making partial duplexes (5\textrm{$^\prime$} to 3\textrm{$^\prime$})\end{tabular}} \\ \hline
Blocking-Cy5full                   & GCTATCTGTTGCTGGCAC
\\ \hline
Blocking-Cy5gap                  & TGGCTATCTGTTGCTGGCAC
\\ \hline
Blocking-Cy3                   & CCCATTCGAGCTCGTTGTAG                             \\ \hline


\end{longtable}
